3DCaricShop: A Dataset and A Baseline Method for Single-view 3D Caricature Face Reconstruction

Caricature is an artistic representation that deliberately exaggerates the distinctive features of a human face to convey humor or sarcasm. However, reconstructing a 3D caricature from a 2D caricature image remains a challenging task, mostly due to the lack of data. We propose to fill this gap by introducing 3DCaricShop, the first large-scale 3D caricature dataset that contains 2000 high-quality diversified 3D caricatures manually crafted by professional artists. 3DCaricShop also provides rich annotations including a paired 2D caricature image, camera parameters and 3D facial landmarks. To demonstrate the advantage of 3DCaricShop, we present a novel baseline approach for single-view 3D caricature reconstruction. To ensure a faithful reconstruction with plausible face deformations, we propose to connect the good ends of the detailrich implicit functions and the parametric mesh representations. In particular, we first register a template mesh to the output of the implicit generator and iteratively project the registration result onto a pre-trained PCA space to resolve artifacts and self-intersections. To deal with the large deformation during non-rigid registration, we propose a novel view-collaborative graph convolution network (VCGCN) to extract key points from the implicit mesh for accurate alignment. Our method is able to generate highfidelity 3D caricature in a pre-defined mesh topology that is animation-ready. Extensive experiments have been conducted on 3DCaricShop to verify the significance of the database and the effectiveness of the proposed method.

==> figures/VC-GCN.tex <==
\begin{figure}% use float package if you want it here
    \begin{center}
    \includegraphics[width=2.5in]{figs/VC-GCN.pdf}
  \caption{}
  \label{fig:VC-GCN}
  \vspace{-4mm}
  \end{center}
\end{figure}

==> figures/fig_failure_case.tex <==
\begin{figure}% use float package if you want it here
    \begin{center}
    \includegraphics[width=2.5in]{figs/exps/failed.png}
  \caption{Failure cases. For some rare exaggerated shapes our framework fail to detect the correct 3D landmarks so that the generated meshes are broken, as the first sample shown. Besides, if the reconstruction of implicit function fails to recover the shape of face features, our framework would suffer from artifacts. }
  \label{fig:failure}
  \vspace{-4mm}
  \end{center}
\end{figure}

==> sections/method_pifu.tex <==
\subsection{3D Modeling using Implicit Function}
\label{sec:pifu}
To capture the diversty of geometric variation in the 3D data, we adopt Pixel-aligned Implicit Function \cite{saito2019pifu} to reconstruct the underlying 3D shape from images. With the strong capability of representation, the implicit function can learn details of the target meshes while trained with the pairs of the target caricature images and the ground truth meshes aligned with the targets. 

\paragraph{Formulation of the reconstruction} We briefly review the method in \cite{saito2019pifu}, which achieves the 3D reconstruction from images by estimating the occupancy of a dense 3D shape, which determines whether a point in 3D space is inside the target model of not. The goal of PIFu is to fit an implicit binary function, $f(\mathbf{X})$. The function maps a given 3D location in continuous camera space $ \mathbf = (\mathbf{X}_x,\mathbf{X}_y,\mathbf{X}_z)\in \mathbb{R}^3$ into the occupancy value.
\begin{equation}
    f(\mathbf{X},\mathbf{I})=\begin{cases}
    1 ,& \text{if} X \text{ is inside mesh surface,}\\
    0, &\text{otherwise.}
    \end{cases}
\end{equation}
where $\mathbf{I}$ is a single RGB image. The function is modelled by a neural network. Specifically, the function $f$ first extracts images features embedding from the projected 2D position at $\pi(\mathbf{X})=\mathbf{x}\in \mathbb{R^2}$, denoted by $\phi (\mathbf{x}, \mathbf{I})$. $\pi$ represents orthogonal projection, and thus $\mathbf{x}=\pi (\mathbf{X})=(\mathbf{X}_x, \mathbf{X}_y)$. After that, the occupanycy of the query $\mathbf{X}$ is estimated, and thus:
\[f(\mathbf{X}, \mathbf{I})=g(\phi(\mathbf{x}, \mathbf{I}),Z)\], where $Z=\mathbf{X}_z$ is the depth along the ray cast by the 2D projection $\mathbf{x}$. Inspired by \cite{saito2020pifuhd}, we further introduce normal maps of the target images to strength the learning capability on local features. We first render the front- and back-view (regrading to the pose of corresponding images) normal maps for our training data, and train a pixel2pixel-hd\cite{wang2018high} to learn the mapping between caricature images and their normal maps. Thus the function $f$ can be written as following: 
\[f(\mathbf{X}, \mathbf{I},\mathbf{F}, \mathbf{B})=g(\phi(\mathbf{x}, \mathbf{I},\mathbf{F}, \mathbf{B}),Z),\] where $\mathbf{F}, \mathbf{B}$ represent the normal maps of front view and back view respectively. $g$ fouces on the varying input depth $Z$ to disambiguate the occupancy of 3D points along the cast rays. Following \cite{saito2019pifu}, a Convolutional Neural Network is used for modelling the function $\phi$ and $g$. 

\paragraph{The training loss} The loss function for the training is the average of mean squared error:
\begin{equation}
    \mathcal{L}=\frac{1}{n}\sum^{n}_{i=1}|f(\mathbf{X}_i, \mathbf{I}_i,\mathbf{F}_i, \mathbf{B}_i)-f^{*}(\mathbf{X}_i)|^{2},
\end{equation}
where $f^{*}(\mathbf{X}_i)$ is value of the ground truth occupancy field. %In the training stage, we follow the samples strategy in PIFu\cite{} to extract training points in the 3D space and set the ground truth value of them.
%During inference, we densely sample the output probability filed over the 3D space and extract the iso-surface with a 0.5 level-set, using the Marching Cube algorithm\cite{lorensen1987marching}. 

==> sections/method_registrations.tex <==
\subsection{Landmark-guided Registration}
\label{sec:registration}

The output meshes $\meshPIFu$ is not topologically uniform. We adopt non-rigid registration\cite{amberg2007optimal} to deform a template $\meshTemp$ into the shape of $\meshPIFu$, in order to unify the topology of our models. As shown in \cite{amberg2007optimal}, Without landmarks the cost function of registration has global minima where the template is collapsed onto a point on the target surface. Thus it's important to introduce the 3D landmark of both meshes to guide the deformation. The process of 3D landmark localization would described in the next section. Since the huge difference between $\meshTemp$ and $\meshPIFu$, the deformation is likely to generate artifacts on meshes, such self-intersection. To resolve this problem, we iteratively perform NICP and PCA projection of the results to obtain $\meshNICP$ and $\meshPCA$. After projection, we obtain a deformed template which is closer to $\meshPIFu$ in shape. Fig. \ref{} illustrates the process of the progressive deformation. 

==> sections/result_application.tex <==
\subsection{Applications}
